Asymptotically Optimal Sampling-Based Path Planning Using Bidirectional Guidance Heuristic

This paper introduces Bidirectional Guidance Informed Trees (BIGIT*),~a new asymptotically optimal sampling-based motion planning algorithm. Capitalizing on the strengths of \emph{meet-in-the-middle} property in bidirectional heuristic search with a new lazy strategy, and uniform-cost search, BIGIT* constructs an implicitly bidirectional preliminary motion tree on an implicit random geometric graph (RGG). This efficiently tightens the informed search region, serving as an admissible and accurate bidirectional guidance heuristic. This heuristic is subsequently utilized to guide a bidirectional heuristic search in finding a valid path on the given RGG. Experiments show that BIGIT* outperforms the existing informed sampling-based motion planners both in faster finding an initial solution and converging to the optimum on simulated abstract problems in $\mathbb{R}^{16}$. Practical drone flight path planning tasks across a campus also verify our results.

==> dead.tex <==
  We proceed this theorem by (1) AWA*'s $Open$ is first translated to an edge queue, $Q^{AWA*}_E$, and then it terminates if there are no edges on $Q^{AWA*}_E$ with f-cost less than the best solution found so far.
  
  AWA* selects best node $s$ from $Open$ with minimal a non-admissible path cost: $\hat{f'}(s) = g(s) + w*\hat{h}(s)$, and g$(s)$ is obtained by: $g(s) = \min_{p\in parent(s)}\{ g(p) + c(p,s)\}$, where parent(s) represents the potential parent of $s$. 
  
  Therefore, AWA*'s edge queue could include:  a state $s$ with its child node $s'$ with $\hat{f'}(s,s') = g(s) + c(s,s') + w*\hat{h}(s')$ for each edge. Then AWA* could select the best edge from: $(s,s') = \argmin_{(s,s') \in Q^{AWA*}_E}\{ \hat{f'}(s,s')\}$. 
  
  AWA* terminates if the goal node $\chi_{goal}$ is with $\min_{(s,s') \in Q^{E}_{AWA*}}\{ g(s) + c(s,s') +\hat{h}(s')\} \geq g(\chi_{goal})$.
  
  This algorithm terminates if for any goal states with $\min_{(s,s') \in Q_{thisgl}}\{ g(s) + \hat{c}(s,s') +h(s')\} \geq g(\chi_{goal})$. This is looser than AWA*, as $\hat{c}$ is admissible. So, this algorithm searches at least all edges that AWA* will be processed. 
  
  
   \begin{algorithm}
 \SetKw{KwOr}{ or }
  \ForEach{$t\in K_{nearest}(s)\{t \in X_{samples} \KwOr t\in V \}$}{
    \eIf{$s \in Expanded \cap t \in V   \cap g(s) +\hat{c}(s,t)< g(t)$}{
           $Q_E \xleftarrow[]{+}\{g(s) + \hat{c}(s,t)+w*\hat{h}(t)\}$;
    }{
      \eIf{$t\in V$}{
        \If{$g(s) +\hat{c}(s,t)< g(t)$}{ $Q_E \xleftarrow[]{+}\{g(s) + \hat{c}(s,t)+w*\hat{h}(t)\}$;}
      }{
         \If{$g(s) + \hat{c}(s,t)+\hat{h}(t) < g(X_{goal})$}{ $Q_E \xleftarrow[]{+}\{g(s) + \hat{c}(s,t)+w*\hat{h}(t)\}$;}
      }
    }
  }
\caption{$ExpandVertex(s,X_{samples})$}
\label{algExpand}
\end{algorithm}

 \begin{algorithm}
  \SetKw{KwOr}{ or }
   \SetKw{KwAnd}{ and }
  $X_{samples} \xleftarrow[]{-}\{s \in X_{samples}|\hat{f}(s) \geq g(X_{goal})\}$;\\
   $V \xleftarrow[]{-}\{s \in V |\hat{f}(s) > g(X_{goal})\}$;\\
    $E \xleftarrow[]{-}\{(s,t) \in E |\hat{f}(s) > g(X_{goal}) \KwOr \hat{f}(t) > g(X_{goal})\}$;\\
     $X_{samples} \xleftarrow[]{+}\{s \in V|s \notin Expanded \KwAnd \hat{f}(s) < g(X_{goal})\}$;\\
    $V \xleftarrow[]{-}\{s \in V |s \notin Expanded\}$;\\
 \caption{$Prune(X_{goal})$}
\label{algPrune}
\end{algorithm}


\begin{table}[h!]
%\small\addtolength{\tabcolsep}{-5.5pt}
\begin{tabular}{ l|rrr}
weights & Random10 & Random20 & Random30  \\ \hline
 AWBIT*(1.2-C1) &   & 0.32   &1284 \\
 AWBIT*(1.5-C1) & 15375.9 & 0.18 & 871 \\
 AWBIT*(1.8-C1) & 15375.9 & 0.26 & 1168 \\
 AWBIT*(2-C1) &15375.9 &0.38 & 1737\\ 
 AWBIT*(3-C1) &15375.9 &0.45 & 1991\\ 
 AWBIT*(5-C1) & 15726.6 & 0.05 & 836 \\
 AWBIT*(10-C1) & 15375.9 & 0.45 & 1991 \\
\end{tabular}
\caption{Comparison of different heuristics.  lengths in meters, times in seconds}
\label{table:1}
\end{table}


\begin{table}[h!]
%\small\addtolength{\tabcolsep}{-5.5pt}
\begin{tabular}{ l|rrr}
weights & Random10(s) & Random20(s) & Random30(s)  \\ \hline
 BIT*(1)       & 3.96083  &19.1356  & 298.275 \\ 
 AWBIT*(1.2-C1) &2.52314  & 12.8961 & 241.502 \\
 AWBIT*(1.5-C1) & 0.79052 & 8.48819 & 188.15 \\
 AWBIT*(1.8-C1) & 0.18432 & 4.59706 & 151.493 \\
 AWBIT*(2-C1) &0.17818    & 2.4393  & 191.849\\ 
 AWBIT*(3-C1) &0.14131    &1.21696  & 41.4515\\ 
 AWBIT*(5-C1) & 0.11674   & 0.80774 & 38.0549 \\
 AWBIT*(10-C1) & 0.13107  & 0.75834  & 31.1572 \\
\end{tabular}
\caption{Comparison of searching time of the first solutions in Random10, Random20 and Random30}
\label{table:1}
\end{table}


==> rootc.tex <==
  \If{$Q_E = \emptyset$}{
   Reset $w$ \tcp*{Case1}
   AddnewSamples;\\ 
   Prune the motion tree;\\
   decrease $w$ \tcp*{Case2}
   Expand($\mathit{Start}$);\\
 }
 \myred{$(s,s') = \argmin_{(s,s')}\{g(s)+\hat{c}(s,s') + w*\hat{h}(s')\}$};\\
 \eIf{$g(s) + \hat{c}(s,s') + \hat{h}(s')<g(X_{goal})$}{
    \If{the edge(s,s') is collision free}{
      compute the true cost of the edge;\\
      update the search tree with the edge;\\
      Expand($s'$);\\
      \If{$s' = X_{goal}$}{
        Set $Q_E$ to be $\emptyset$ \tcp*{Case2}
        decrease $w$ \tcp*{Case1} 
        \myblue{Online Prediction} \tcp*{Case1}
      }
    }
 } {
   If $w>1:$ decrease $w$ \tcp*{Case1}
   If{ $w<=1$: } \tcp*{Case1}
   Set $Q_E$ to be $\emptyset$;
 }
 
 Theorem~\ref{t1} proves that at least all edges searched by \algname\ will have been processed by AWA* for a given RGG when decreasing weights on the same batch. 
\begin{theorem}\label{t1}
For a given RGG, at least all edges consists of the motion tree generated by \algname\ would be searched by AWA*. 
\end{theorem}
\begin{proof}
 We proceed this theorem by (1) AWA*'s $Open$ is first translated to an edge queue, $Q^{AWA*}_E$, and then it terminates if there are no edges on $Q^{AWA*}_E$ with f-cost less than the best solution found so far.
  
  AWA* selects best node $s$ from $Open$ with minimal a non-admissible path cost: $\hat{f'}(s) = g(s) + w*\hat{h}(s)$, and g$(s)$ is obtained by: $g(s) = \min_{p\in parent(s)}\{ g(p) + c(p,s)\}$, where parent(s) represents the potential parent of $s$. 
  
  Therefore, AWA*'s edge queue includes:  a state $s$ with its child node $s'$ with $\hat{f'}(s,s') = g(s) + c(s,s') + w*\hat{h}(s')$ for each edge. Then AWA* selects the best edge from: $(s,s') = \argmin_{(s,s') \in Q^{AWA*}_E}\{ \hat{f'}(s,s')\}$. 
  
  AWA* terminates if the goal node $X_{goal}$ is with $\min_{(s,s') \in Q^{E}_{AWA*}}\{ g(s) + c(s,s') +\hat{h}(s')\} \geq g(X_{goal})$.
  
  \algname\ terminates if for any goal states with $\min_{(s,s') \in Q_{thisgl}}\{ g(s) + \hat{c}(s,s') +h(s')\} \geq g(X_{goal})$. This is looser than AWA*, as $\hat{c}$ is admissible. So, this algorithm searches at least all edges that AWA* will be processed. 
\end{proof}
\begin{theorem}
 \algname\ will almost-surely converge to an optimal path, if this path exists, as the additional number of states, $q$, goes to infinity, i.e..
  \begin{align*}
      P(\lim_{p\to\infty}supC^{AWBIT^*}_{best,q} = C^*) = 1,
  \end{align*}
\end{theorem}
\begin{proof}
\algname\ selects the best edge and updates the cost to come of each state with the same condition as AWA*, so \algname\ finds an optimal solution. Therefore, when the number of samples reaches infinity, \algname\ almost-surely asymptotically finds an optimal path. 
\end{proof}

Theorem~\ref{t3} proves that at least all edges searched by \algname\ will have been processed by BIT* for a given RGG after weight decreases to 1 when decreasing weight for adding new samples. 

\begin{theorem} \label{t3}
 After weight decreases to 1, \algname\ will maintain the following property as BIT* for each new batch of samples:
 \begin{align*}
      P(\lim_{p\to\infty}supC^{AWBIT^*}_{best,q} = C^*) = 1,
 \end{align*}
\end{theorem}
\begin{proof}
 When the weight decreases to 1, the edge queue, $Q_E$, for \algname\ is to be in order of admissible estimated total cost for any edge, that is, \algname\ employs admissible heuristic to search, which follows the same property as BIT*. So, after \algname\ restarts a new search, each expanded vertex $s$ will connect its best $k$-neighbors if they could provide a better solution. Edges to unconnected samples and connected samples that was on the tree always are inserted into $Q_E$, which are the same process as BIT*. Then \algname\ employs the same edge process as BIT*, so there are no difference that is different from asymptotic optimality of BIT*:
 \begin{align*}
    P(\lim_{p\to\infty}supC^{BIT^*}_{best,q} = C^*) = 1.
 \end{align*}
  Therefore \algname\ maintains asymptotic optimality after the weight decreases to 1.
\end{proof}
and $\mathbf{t}$ is on the $Open$ of the opposite search tree,
 and $\mathbf{t}$ be on $Open$ of the forward search tree
 and $\widehat{g}_{\mathcal{F}}(\mathbf{t}) \leq g_{\mathcal{F}}(\mathbf{t}) \leq \frac{1}{2}C_{best}$
 +\widehat{c}(\mathbf{s},\mathbf{t})
 and $\mathbf{t}$ with
 and $\mathbf{t}$ with
 +c(\mathbf{s},\mathbf{t})
 
   \label{fig:biit}
   
   
   
             \begin{tikzpicture}
% \filldraw[green!20] (1,2) -- (6,2) -- (6,0)--(3,0) --cycle;  
  %\filldraw[cyan!40] (4,1) -- (6,1/3) -- (6,0)--(4,0) --cycle;  
\draw[thick] (0,0) -- (7,0) node[anchor=north west]{};
\draw[thick] (0,0) -- (0,3) node[anchor=south east]{};
\draw[thick] (0,3) -- (7,3) node[anchor=south east]{};
\draw[thick] (7,0) -- (7,3) node[anchor=south east]{};

\filldraw[gray] (3,0) rectangle(4,2.5);
%\draw[step=1cm,gray,thick](0,0) grid(7,3);
%\foreach \x in {0,...,7}
  %\draw (\x cm,1pt) -- (\x cm,-1pt) node[anchor=north] {$\x$};
%\foreach \y in {1,2,3}
  %\draw (1pt,\y cm) -- (-1pt,\y cm) node[anchor=east] {$\y$};
  %\draw[dashed] (1.5,1.5) -- (1.65,0.65); 
  %\draw[dashed] (1.5,1.5) -- (2.7,1.8); 
   %\draw[dashed] (1.5,1.5) -- (1.9,2); 
    %\draw[dashed] (1.5,1.5) -- (2.6,0.8); 
  %\draw[dashed] (1.5,1.5) -- (0.9,1.3); 
   %\draw[dashed] (1.5,1.5) -- (1.1,2.1); 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %\draw[dashed] (5.5,1.5) -- (4.6,1.9); 
  %\draw[dashed] (5.5,1.5) -- (4.7,1.1); 
   %\draw[dashed] (5.5,1.5) -- (5.2,0.7); 
    %\draw[dashed] (5.5,1.5) -- (6.2,0.6); 
  %\draw[dashed] (5.5,1.5) -- (6.1,2.05); 
   %\draw[dashed] (5.5,1.5) -- (5.4,2.45); 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %\draw[dashed] (0.7,0.3) -- (1.65,0.65); 
  %\draw[dashed] (0.7,0.3) -- (0.9,1.3); 
   %\draw[dashed] (0.7,0.3) -- (1.5,1.5); 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %\draw[dashed] (2.6,0.8) -- (1.65,0.65); 
  %\draw[dashed] (2.6,0.8) -- (2.7,1.8); 
    %\draw[dashed] (1.65,0.65) -- (2.7,1.8); 
   %\draw[dashed] (0.9,1.3) -- (1.65,0.65); 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %\draw[dashed] (1.1,2.1) -- (0.4,2.6); 
    %\draw[dashed] (1.1,2.1) -- (0.9,1.3); 
   %\draw[dashed] (1.1,2.1) -- (1.9,2); 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  %\draw[dashed] (1.1,2.1) -- (0.4,2.6); 
    %\draw[dashed] (2.52,2.58) -- (1.9,2); 
   %\draw[dashed] (2.7,1.8) -- (1.9,2); 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \draw[green,dashed,thick] (5.5,1.5) -- (4.6,1.9); 
  \draw[red!50!yellow,thick] (4,2.5) -- (4.6,1.9); 
   \draw[red!50!yellow,thick] (4.7,1.1) -- (4.6,1.9); 
     \draw[red!50!yellow,thick] (4,2.5) -- (4.4,2.57);
       \draw[red!50!yellow,thick] (4,2.5) -- (5.4,2.45); 
\draw[green,dashed,thick] (5.5,1.5) -- (5.4,2.45);       \draw[green,dashed,thick] (5.5,1.5) -- (4.7,1.1); 
   \draw[blue,thick] (2.52,2.58) -- (1.9,2); 
   \draw[blue,thick] (3.5,2.9) -- (4,2.5); 
   \draw[blue,thick] (4,2.5) -- (2.52,2.58); 
    \draw[blue,thick] (4,2.5) -- (2.7,1.8); 
    \draw[green,dashed,thick] (2.7,1.8) -- (1.5,1.5); 
      \draw[green,dashed,thick] (2.6,0.8) -- (1.5,1.5); 
  \draw[blue,thick] (2.7,1.8) -- (2.6,0.8); 
   \draw[green,dashed,thick] (1.5,1.5) -- (1.9,2); 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\filldraw[red] (5.5,1.5) circle (2.5pt);
\filldraw[green] (1.5,1.5) circle (2.5pt);
\filldraw[black] (2.6,0.8) circle (2pt);
\filldraw[black] (0.7,0.3) circle (2pt);
\filldraw[black] (1.65,0.65) circle (2pt);
\filldraw[black] (2.7,1.8) circle (2pt);
\filldraw[black] (1.9,2) circle (2pt);
\filldraw[black] (2.52,2.58) circle (2pt);
\filldraw[black] (0.4,2.6) circle (2pt);
\filldraw[black] (0.9,1.3) circle (2pt);
\filldraw[black] (1.1,2.1) circle (2pt);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\filldraw[black] (3.5,2.9) circle (2pt);
\filldraw[black] (4,2.5) circle (2pt);
\filldraw[black] (4.4,2.57) circle (2pt);
\filldraw[black] (4.6,1.9) circle (2pt);
\filldraw[black] (4.7,1.1) circle (2pt);
\filldraw[black] (4.75,0.3) circle (2pt);
\filldraw[black] (5.2,0.7) circle (2pt);
\filldraw[black] (6.2,0.6) circle (2pt);
\filldraw[black] (6.7,1.1) circle (2pt);
\filldraw[black] (5.4,2.45) circle (2pt);
\filldraw[black] (6.8,2.9) circle (2pt);
\filldraw[black] (6.1,2.05) circle (2pt);
\end{tikzpicture}  


  BIT* is asymptotically optimal when an admissible heuristic serves, because selecting implicit edges to build a motion tree growing from a start state to the goal state by in order of increasing estimated total path cost through these edges with the respect to the number of samples is similar to an edge-queue version of LPA*. So, if a more accurate and admissible heuristic than Euclidean norm is provided to BIT*, the path length for each batch should not be larger than BIT* with Euclidean norm while it also improves the searching time, especially for the first solution. Otherwise, the heuristic cannot be guaranteed to be admissible.   
  
  
  The assumption for backward search tree is analogous. Then we will have $\widehat{g}_\mathcal{B}(\mathbf{s}) \leq g_\mathcal{B}(\mathbf{s}) \leq \frac{1}{2}C_{best}$ and  $\widehat{g}_{\mathcal{F}}(\mathbf{s}) \leq g_{\mathcal{F}}(\mathbf{s}) \leq \frac{1}{2}C_{best}$.
 
  Consider $\mathbf{s}$ with $\widehat{g}_\mathcal{B}(\mathbf{s}) +\widehat{g}_\mathcal{F}(\mathbf{s}) \leq g_{\mathcal{B}}(\mathbf{s}) +g_{\mathcal{F}}(s)$. We distinguish two cases to use the consistency of $\widehat{h}_{\mathcal{F}}(\mathbf{s}) = \widehat{g}_\mathcal{B}(\mathbf{s})$ and $\widehat{h}_\mathcal{B}(\mathbf{s}) = \widehat{g}_\mathcal{F}(\mathbf{s})$.
  
  Case1: For a state $\mathbf{s'}$ on $Open_\mathcal{F}$(one of $k$-nearest neighbors of $\mathbf{s}$), $\mathbf{s}$ is the nearest expanded state of the backward search tree. That is, $\widehat{g}_\mathcal{B}(\mathbf{s}) =\widehat{h}_\mathcal{F}(\mathbf{s})$ is the lower bound of all h-values of the expanded states on the backward search tree for $\mathbf{s}$. Because $\widehat{g}_\mathcal{B}(\mathbf{s}) \leq g_\mathcal{B}(\mathbf{s}) = h_\mathcal{F}(\mathbf{s})$, so we will have:
 \begin{align*}
     \widehat{h}_\mathcal{F}(\mathbf{s'}) &= \widehat{c}(\mathbf{s'},\mathbf{s}) + \widehat{g}_\mathcal{B}(\mathbf{s})\\ &\leq c(\mathbf{s'},\mathbf{s}) +g_\mathcal{B}(\mathbf{s})\\
     &= c(\mathbf{s'},\mathbf{s}) + h_\mathcal{F}(\mathbf{s});%
 \end{align*}
  We know $\widehat{h}_\mathcal{F}(\mathbf{s'}) = c(\mathbf{s'},\mathbf{s}) + h_\mathcal{F}(\mathbf{s})$ denotes consistent heuristic. This is, $\widehat{h}_\mathcal{F}(\mathbf{s'})$ is admissible. Then in the same way, for any state $\mathbf{v}$ with $\widehat{g}_\mathcal{F}(\mathbf{v})$ on the forward search tree, after updating heurisitic from $\mathbf{s}$ to $\mathbf{v}$, we will have:
  \begin{align*}
      \widehat{h}_\mathcal{F}(\mathbf{v}) &= d(\mathbf{v},\mathbf{s}) + \widehat{h}_\mathcal{F}(\mathbf{s}) \leq c^*(\mathbf{v},\mathbf{s}) +h_\mathcal{F}(\mathbf{s}) = h_\mathcal{F}(\mathbf{v}).
  \end{align*}
   where $d(\mathbf{v},\mathbf{s})$ denotes the minimum estimated path cost from $\mathbf{s}$ to $\mathbf{v}$.  So, we know the heuristic value for $\mathbf{v}$ is also admissible.
   
  Case2: For a state $\mathbf{s''}$(one of $k$-nearest neighbors of $\mathbf{s}$) on $Open_\mathcal{B}$, $\mathbf{s}$ is the nearest expanded state with $\widehat{g}_\mathcal{F}(\mathbf{s}) \leq g_\mathcal{F}(\mathbf{s}) = h_\mathcal{B}(\mathbf{s})$ on the forward search tree. That is, $\widehat{g}_\mathcal{F}(\mathbf{s}) =\widehat{h}_\mathcal{B}(\mathbf{s})$ is the lower bound of all h-values of the expanded states on the forward search tree for $\mathbf{s}$. So, we will have:
  \begin{align*}
      \widehat{h}_\mathcal{B}(\mathbf{s''}) &= \widehat{c}(\mathbf{s''},\mathbf{s}) + \widehat{g}_\mathcal{F}(\mathbf{s}) \\ &\leq c(\mathbf{s''},\mathbf{s}) +g_\mathcal{F}(\mathbf{s}) \\
      &= c(\mathbf{s''},\mathbf{s}) + h_\mathcal{B}(\mathbf{s});%
  \end{align*}
    We know $ \widehat{h}_\mathcal{B}(\mathbf{s''}) \leq c(\mathbf{s'},\mathbf{s}) + h_\mathcal{F}(\mathbf{s})$ represents the consistent heuristic. This is, $\widehat{h}_\mathcal{B}(\mathbf{s''})$ is admissible. In the same way, we will then have $\widehat{h}_\mathcal{B}(\mathbf{v'}) \leq c^*(\mathbf{v'},\mathbf{s}) + h_\mathcal{B}(\mathbf{v'}) \leq h_\mathcal{B}(\mathbf{v'})$ for $\mathbf{v'}$ with $\widehat{g}_\mathcal{B}(v')$ on backward search tree. 


    %%%%%%%%%%
   In this paper,  Bidirectionally Informed Trees (BiIT*), an asymptotically optimal sampling-based motion planning algorithm based on the bidirectional graph search and informed sampling-based planning. For given batch of samples representing as an implicit random geometric graph (RGG), BiIT* is able to integrate the efficient nature of bidirectional graph search techniques, such as Meet in Middle (MM), with anytime informed sampling-based algorithms, such as Batch Informed trees (BIT*).

BiIT* employs an accurate and provably admissible bidirectional heuristic by adapting to bidirectional heuristic search to update heuristic without collision checking to search on a given RGG from start and goal states towards each other simultaneously while it reuses the information of previous search. It can be treated as running BIT* with a more accurate heuristic in both directions in a continuous state space from the start and goal states simultaneously. It is showed that BiIT* is probabilistically complete and asymptotically optimal.

Dijkstra's algorithm is then applied to that state for obtaining the admissible heuristic, with forward and reverse search respectively. By using our provided condition, the search time is greatly reduced.

We further give a condition with the  



Dijkstra's algorithm with our provided condition is then applied to update heuristic from that state towards the start and goal respectively. Once the start and goal are found by Dijkstra's algorithm with our provided condition, an accurate and admissible heuristic is provided.

The possible heuristic choice range is then limited greatly reduced by using a proposed condition .

An accurate and provably admissible heuristic is then provided for any state already generated by the bidirectional search by Dijkstra's algorithm subjected to upper admissible cost. BiIT* uses the provided precise and admissible heuristic to search an increasingly dense implicit random geometric graph by an incrementally bidirectional search. The process is considered as running BIT* with the accurate heuristic in both directions in a continuous state space from the start and goal states simultaneously. 
 In other words, there must exist a state $\mathbf{s}$, satisfying $U \leq max(C,f_{minF},fminB,gminF+gminB+\epsilon)$, to stop the search without collision checking, where $U = \widehat{g}_\mathcal{B}(\mathbf{s})  +\widehat{g}_\mathcal{F}(\mathbf{s}) \leq U_{\mathbf{E}}$. Namely,  $\widehat{g}_\mathcal{F}(s)$ and $\widehat{g}_\mathcal{B}(s)$ provide the lower cost-to-go bound for reverse and forward search trees respectively except other middlers. 

 
 A monotone/consistent heuristic $h$ satisfies the triangle inequality, $h(\mathbf{u}) \leq k(\mathbf{u},\mathbf{v})+h(\mathbf{v})$ for any pair of states $\mathbf{u}$ and $\mathbf{v}$, where $k(\mathbf{u},\mathbf{v})$ represents the least path cost from $\mathbf{u}$ to $\mathbf{v}$~\cite{Pearl}. Note that every consistent heuristic is admissible.

%In this paper, we investigate a novel asymptotically optimal sampling-based motion planning algorithm -- Bidirectionally Informed Trees (BiIT*). The algorithm integrates the intrinsic efficiency of bidirectional heuristic search with the anytime informed sampling-based algorithm. An accurate and admissible heuristic can be guaranteed by using a lazy bidirectional search with a lazily enhanced Dijkstra's algorithm for bidirectional search. It can be treated as running BIT* with the provided accurate heuristic in both directions in a continuous state space from the start and goal states simultaneously. It show that BiIT* is probabilistically complete and asymptotically optimal. 

%It can be treated as running BIT* with the provided accurate heuristic in both directions in a continuous state space from the start and goal states simultaneously.


Batch Informed Trees(BIT*) is an anytime algorithm combining strengths of heuristic search and anytime sampling-based planner by employing heuristic to find an optimal solution for batch of informally sampled states representing as an increasingly dense implicit random geometric graph(RGG)~\cite{rgg}. 

, but RRT-connect neither concentrates on the solution quality nor get better solutions with additional time


  BIT*~\cite{bit}, an asymptotically optimal sampling-based motion planning algorithm, employs an admissible heuristic to quickly find an optimal initial solution with respect to the number of sampled states representing as RGG. It then provides the new states that could possibly provide a better solution than the current path cost by informed sampling, and gets better and better solutions with additional states until it converges to an optimal solution or time expires.

     Let $\mathcal{T_F}:=(V_\mathcal{F},E_\mathcal{F})$ and $\mathcal{T_\mathcal{B}}:=(V_\mathcal{B},E_\mathcal{B})$ be the explicit forward and reverse trees with the set of states, $\{V_\mathcal{F}, V_\mathcal{B}\} \subset X_{free}$, and edges, $E_\mathcal{F} = \{(\mathbf{u}_{\mathcal{F}},\mathbf{v}_{\mathcal{F}} ) | \{\mathbf{u}_{\mathcal{F}},\mathbf{v}_{\mathcal{F}}\} \in V_{\mathcal{F}} \ \}$ and $E_\mathcal{B} = \{(\mathbf{u}_{\mathcal{B}},\mathbf{v}_{\mathcal{B}} ) | \{\mathbf{u}_{\mathcal{B}},\mathbf{v}_{\mathcal{B}}\} \in V_{\mathcal{B}} \ \}$, where $\mathbf{u}$ is the parent state of $\mathbf{v}$, respectively.  
   
   The function $\widehat{g}_\mathcal{F}(\mathbf{x})$ and $\widehat{g}_\mathcal{B}(\mathbf{x})$ denote the admissible estimates of the cost-to-come to state $\mathbf{x}$, $\mathbf{x} \in X_{free}$, from $X_{start}$ and from $X_{goal}$ respectively. $g_{\mathcal{F}}(\mathbf{x})$ and $g_{\mathcal{B}}(\mathbf{x})$ represent the true cost-to-come to $\mathbf{x}$ from $X_{start}$ or $X_{goal}$ given the current forward and backward search tree.  $\overline{g}_{\mathcal{F}}(\mathbf{x})$ and $\overline{g}_{\mathcal{B}}(\mathbf{x})$ represent the lower admissible cost-to-come bound, such as Euclidean norm, to state $\mathbf{x}$ from $X_{start}$ and $X_{goal}$ respectively. It is important to realize that
   $\overline{g}_\mathcal{F}(\mathbf{x})\leq \widehat{g}_\mathcal{F}(\mathbf{x}) \leq g_\mathcal{F}(\mathbf{x})$ and $\overline{g}_\mathcal{B}(\mathbf{x})\leq \widehat{g}_\mathcal{B}(\mathbf{x}) \leq g_\mathcal{B}(\mathbf{x})$, respectively. 
   
   The function $\widehat{h}_\mathcal{F}(\mathbf{x})$ and $\widehat{h}_\mathcal{B}(\mathbf{x})$ represent the admissible estimates of the cost-to-go from a sate $\mathbf{x}$, $\mathbf{x} \in X_{free}$, to the goal and to the start respectively. $h_{\mathcal{F}}(\mathbf{x})$ and $h_{\mathcal{B}}(\mathbf{x})$ denote the cost-to-go from $\mathbf{x}$ to $X_{start}$ and $X_{goal}$ given the current forward and backward search tree. $\overline{h}_{\mathcal{F}}(\mathbf{x})$ and $\overline{h}_{\mathcal{B}}(\mathbf{x})$ represent the lower admissible cost-to-go bound, such as Euclidean norm, from state $\mathbf{x}$ to $X_{goal}$ and $X_{start}$ respectively. It is essential to recognize $\overline{h}_\mathcal{F}(\mathbf{x})\leq \widehat{h}_\mathcal{F}(\mathbf{x}) \leq h_\mathcal{F}(\mathbf{x})$ and $\overline{h}_\mathcal{B}(\mathbf{x})\leq \widehat{h}_\mathcal{B}(\mathbf{x}) \leq h_\mathcal{B}(\mathbf{x})$, respectively.
   
   It is important to recognize that $h_\mathcal{F}(\mathbf{x}) = g_\mathcal{B}$ ,$\widehat{h}_\mathcal{F}(\mathbf{x}) = \widehat{g}_\mathcal{B} (\mathbf{x})$, and $\overline{h}_\mathcal{F}(\mathbf{x}) = \overline{g}_\mathcal{B}(\mathbf{x})$.

   \textbf{Inadmissible heuristic} provided from reverse search of EIT* and AIT*(a) and admissible heuristic served from bidirectional search of BiIT*(b). Informed trees, such as BIT*, AIT* and EIT*, devote to approximate the searching state space via batches of randomly sampling states(black nodes), which depict a random geometric graph with implicit edges(connections by dots between any two states). These implicit edges are selected to build a motion tree from the start to goal states by in order of increasing estimated total path cost via a heuristic $\mathit{cost}$-$\mathit{to}$-$\mathit{go}$ (color thick dashed lines). The accuracy of heuristic directly affects the searching performance of an algorithm. A $\mathit{priori}$ heuristic, such as Euclidean norm provides the lower bound heuristic, is admissible but inaccurate. The initial solution found by BIT* used Euclidean norm as its heuristic is shown in green ($\textcolor{green}{-}$) (a). AIT* and EIT* provide a more accurate heuristic but cannot guarantee \textbf{admissible} at current approximation of the specific domain (See the analysis in Section~\ref{inadmissible}). The green (\textcolor{green}{$\bullet$}) and the red  (\textcolor{red}{${\bullet}$}) denotes the locations of start and goal states, separately. The initial solutions found by AIT* and EIT* are shown in green ($\textcolor{green}{-}$) and blue ($\textcolor{blue}{-}$) respectively. By employing a lazy bidirectional search and uniform-cost search, BiIT* is able to provide a more precise and an provably bidirectionally admissible heuristic. The initial solution found by BiIT* is shown in blue ($\textcolor{blue}{-}$). In Figure(a), the heuristic provided from reverse tree of AIT* and EIT* is show in dashed orange($\textcolor{orange}{--}$). In Figure(b), the heuristic provided by lazy reverse search of BiIT* is shown in purple($\textcolor{purple}{--}$) while orange($\textcolor{orange}{--}$) presents the heuristic provided by lazy forward search of BiIT*. Figure(a) and (b) are obstained by running BIT*, EIT*, AIT*, and BiIT* on OMPL.

   AIT* and EIT* have the same three high-level procedures: (1) they uniformly incrementally sample batches of states in by informed sampling. (2) They update heuristics by a reverse research that uses a heuristic search from the goal state to the start state for the currently given RGGs without collision checking. (3) They return the collision-free path by forward heuristic search with the provided heuristic updated by the inexpensive reverse search on the current RGGs. For a given RGG, if the reverse search cannot reach the start state, the a new batch of samples will be added to the current RGG.
    In this paper, we investigate an asymptotically optimal sampling-based motion planning algorithm -- Bidirectionally Informed Trees (BiIT*). Unlike asymmetric bidirectional sampling-based planners, such as Effort Informed Trees (EIT*), BiIT* provides an accurate and provably admissible heuristic to direct a bidirectional search of an increasingly dense implicit random geometric graph (RGG) to find an asymptotically optimal solution. BiIT* firstly applies a lazy bidirectional search (without collision-checks) to a given RGG until finding a state that satisfies the stop condition similar to Meet-in-Middle (MM). Then, BiIT* employs a lazy uniform-cost search (such as Dijkstra's algorithm) with a bounded estimated total path cost to update the heuristic for a generated state  from the state of fulfilling the stop condition to the start and goal, respectively. Finally, the provided heuristic is used to induct a bidirectional search for the given RGG. BiIT* is asymptotic completeness and optimality.
 Experimental results show BiIT* outperforms the existing sampling-based motion planners both in faster finding an initial solution and converging to the optima on simulated abstract problems in $\mathbb{R}^8$ and $\mathbb{R}^{16}$ and on UNH-Hover System.

 %The accuracy of a heuristic and an inexpensive edge evaluation can directly refine the anytime profile of an sampling-based motion planner, like AIT* and EIT*~\cite{EIT}. AIT* and EIT* provide an adaptive heuristic by updating heuristic using a reverse search from a goal to a start. The accurate heuristic improves the anytime search performance. However, AIT* and EIT* cannot theoretically guarantee providing the admissible heuristic, although they claim it (analyzes in ~\ref{inadmissible}).


, which consists of a hollow, narrow, and axis-aligned hyper-rectangle enclosing the goal state with a wall gap

 where AIT* claims it provides an admissible heuristic by the reverse search when edge is connected either by k-nearest neighbors or radius, and the calculated admissible heuristic of EIT* is obtained by combining a $\mathit{priori}$ admissible cost heuristic $\hat{c}(\cdot,\cdot)$ with admissible heuristic got from a reverse tree between each state and goal

  Unlike asymmetric bidirectional sampling-based planners, such as Effort Informed Trees (EIT*), BiIT* provides an accurate and provably admissible heuristic to guide a bidirectional search on an increasingly dense implicit random geometric graph (RGG). 











  \begin{figure}[t]
  \vspace{-4mm}
    \centering
    \subfloat[Adaptive heuristic(EIT*)]{
    \scalebox{0.38}{
       \begin{tikzpicture}  
      %\filldraw[green!20] (1,2) -- (6,2) -- (6,0)--(3,0) --cycle; 
           %\filldraw[blue!20] (4,1) -- (6,1/3) -- (6,0)--(4,0) --cycle; 
\draw[ultra thick] (0,0) -- (10,0) node[anchor=north west]{};
\draw[ultra thick] (0,0) -- (0,10) node[anchor=south east]{};
\draw[ultra thick] (0,10) -- (10,10) node[anchor=south east]{};
\draw[ultra thick] (10,0) -- (10,10) node[anchor=south east]{};

\filldraw[gray, ultra thick](4,0) rectangle (6,5.8);
\filldraw[gray, ultra thick](4,6.2) rectangle (6,8);
\filldraw[gray, ultra thick](4,0) rectangle (6,5.8);

0 is expanded. 
	 neighbor -> 14
\draw[thick,dotted,gray] (8,5)--
(9.37629,4.48826);
	 neighbor -> 7
\draw[thick,dotted,gray] (8,5)--
(8.68801,3.30839);
	 neighbor -> 3
\draw[thick,dotted,gray] (8,5)--
(9.78223,4.55585);
	 neighbor -> 18
\draw[thick,dotted,gray] (8,5)--
(9.51248,3.48756);
	 neighbor -> 31
\draw[thick,dotted,gray] (8,5)--
(6.59233,6.6171);
	 neighbor -> 9
\draw[thick,dotted,gray] (8,5)--
(6.72317,6.94032);
	 neighbor -> 26
\draw[thick,dotted,gray] (8,5)--
(6.84629,7.36674);
	 neighbor -> 25
\draw[thick,dotted,gray] (8,5)--
(6.56972,2.59136);
	 neighbor -> 17
\draw[thick,dotted,gray] (8,5)--
(4.82637,6.13703);
	 neighbor -> 23
\draw[ultra thick,dashed,red!50!yellow] (8,5)--
(9.86223,7.9357);

1 is expanded. 
	 neighbor -> 30
\draw[thick,dotted,gray] (2,5)--
(1.43628,4.47904);
	 neighbor -> 19
\draw[thick,dotted,gray] (2,5)--
(2.76515,4.46506);
	 neighbor -> 5
\draw[thick,dotted,gray] (2,5)--
(0.867434,4.19372);
	 neighbor -> 28
\draw[thick,dotted,gray] (2,5)--
(1.53739,6.49119);
	 neighbor -> 2
\draw[thick,dotted,gray] (2,5)--
(2.27339,3.18972);
	 neighbor -> 6
\draw[thick,dotted,gray] (2,5)--
(0.159104,5.27765);
	 neighbor -> 15
\draw[thick,dotted,gray] (2,5)--
(3.8465,3.57475);
	 neighbor -> 24
\draw[thick,dotted,gray] (2,5)--
(3.43305,3.00339);
	 neighbor -> 11
\draw[thick,dotted,red!50!yellow] (2,5)--
(2.62584,7.50763);
	 neighbor -> 23

\draw[ultra thick,dashed,red!50!yellow] (2.62584,7.50763)--
(1.43628,4.47904);
	 neighbor -> 4
\draw[thick,dotted,gray] (2,5)--
(3.08013,2.63871);
	 neighbor -> 8
\draw[thick,dotted,gray] (2,5)--
(3.92942,6.7433);
	 neighbor -> 13
\draw[thick,dotted,gray] (2,5)--
(1.74053,7.90764);
	 neighbor -> 17
\draw[ultra thick,dashed,red!50!yellow] (8,5)--
(4.82637,6.13703);


1  19
19 is expanded. 

	 neighbor -> 30
\draw[ultra thick,dashed,red!50!yellow] (2.76515,4.46506)--
(1.43628,4.47904);
	 neighbor -> 2
\draw[ultra thick,dashed,red!50!yellow] (2.76515,4.46506)--
(2.27339,3.18972);
	 neighbor -> 15
\draw[thick,dotted,gray] (2.76515,4.46506)--
(3.8465,3.57475);
	 neighbor -> 24
\draw[thick,dotted,gray] (2.76515,4.46506)--
(3.43305,3.00339);
	 neighbor -> 4
\draw[thick,dotted,gray] (2.76515,4.46506)--
(3.08013,2.63871);
	 neighbor -> 5
\draw[ultra thick,,dashed,red!50!yellow] (2.76515,4.46506)--
(0.867434,4.19372);
	 neighbor -> 28
\draw[ultra thick,dashed,red!50!yellow] (2.76515,4.46506)--
(1.53739,6.49119);
	 neighbor -> 8
\draw[thick,dotted,gray] (2.76515,4.46506)--
(3.92942,6.7433);
	 neighbor -> 17
\draw[thick,dotted,gray] (2.76515,4.46506)--
(4.82637,6.13703);

	 neighbor -> 17
\draw[ultra thick,dashed,red!50!yellow] (2.76515,4.46506)--
(4.82637,6.13703);



	 neighbor -> 9
\draw[thick,dotted,gray] (6.59233,6.6171)--
(6.72317,6.94032);
	 neighbor -> 26
\draw[thick,dotted,gray] (6.59233,6.6171)--
(6.84629,7.36674);
	 neighbor -> 17
\draw[thick,dotted,gray] (6.59233,6.6171)--
(4.82637,6.13703);
	 neighbor -> 0
\draw[thick,dotted,gray] (6.59233,6.6171)--
(8,5);
	 neighbor -> 29
\draw[thick,dotted,gray] (6.59233,6.6171)--
(5.57414,8.68532);
	 neighbor -> 8
\draw[thick,dotted,gray] (6.59233,6.6171)--
(3.92942,6.7433);

	 neighbor -> 14
\draw[thick,dotted,gray] (6.59233,6.6171)--
(9.37629,4.48826);
	 neighbor -> 23
\draw[thick,dotted,gray] (6.59233,6.6171)--
(9.86223,7.9357);
	 neighbor -> 3
\draw[thick,dotted,gray] (6.59233,6.6171)--
(9.78223,4.55585);
	 neighbor -> 7
\draw[thick,dotted,gray] (6.59233,6.6171)--
(8.68801,3.30839);
	 neighbor -> 25
\draw[thick,dotted,gray] (6.59233,6.6171)--
(6.56972,2.59136);

	 neighbor -> 0
\draw[thick,dotted,gray] (6.59233,6.6171)--
(8,5);

\draw[ultra thick,dashed,red!50!yellow] (8,5)--
(6.59233,6.6171);

9 is expanded. 



	 neighbor -> 29
\draw[ultra thick,dashed,red!50!yellow] (6.72317,6.94032)--
(5.57414,8.68532);

 
	 neighbor -> 27
\draw[ultra thick,dashed,red!50!yellow] (6.72317,6.94032)--
(4.89423,9.53991);
	 neighbor -> 23
\draw[thick,dotted,gray] (6.72317,6.94032)--
(9.86223,7.9357);
	 neighbor -> 14
\draw[thick,dotted,gray] (6.72317,6.94032)--
(9.37629,4.48826);
	 neighbor -> 3
\draw[thick,dotted,gray] (6.72317,6.94032)--
(9.78223,4.55585);


\draw[ultra thick,dashed,red!50!yellow] (6.72317,6.94032)--
(8,5);

25 is expanded. 
	 neighbor -> 7
\draw[thick,dotted,gray] (6.56972,2.59136)--
(8.68801,3.30839);

	 neighbor -> 18
\draw[thick,dotted,gray] (6.56972,2.59136)--
(9.51248,3.48756);
	 neighbor -> 20
\draw[thick,dotted,gray] (6.56972,2.59136)--
(9.57914,1.79577);

	 neighbor -> 14
\draw[thick,dotted,gray] (6.56972,2.59136)--
(9.37629,4.48826);

	 neighbor -> 3
\draw[thick,dotted,gray] (6.56972,2.59136)--
(9.78223,4.55585);

	 neighbor -> 31
\draw[thick,dotted,gray] (6.56972,2.59136)--
(6.59233,6.6171);

	 neighbor -> 0
\draw[ultra thick,dashed,red!50!yellow] (6.56972,2.59136)--
(8,5);

26 is expanded. 

	 neighbor -> 29
\draw[thick,dotted,gray] (6.84629,7.36674)--
(5.57414,8.68532);


	 neighbor -> 27
\draw[thick,dotted,gray] (6.84629,7.36674)--
(4.89423,9.53991);

	 neighbor -> 23
\draw[thick,dotted,gray] (6.84629,7.36674)--
(9.86223,7.9357);


	 neighbor -> 0
\draw[ultra thick,,dashed,red!50!yellow] (6.84629,7.36674)--
(8,5);

14 is expanded. 

	 neighbor -> 18
\draw[thick,dotted,gray] (9.37629,4.48826)--
(9.51248,3.48756);
	 neighbor -> 7
\draw[thick,dotted,gray] (9.37629,4.48826)--
(8.68801,3.30839);

	 neighbor -> 20
\draw[thick,dotted,gray] (9.37629,4.48826)--
(9.57914,1.79577);

	 neighbor -> 23
\draw[thick,dotted,gray] (9.37629,4.48826)--
(9.86223,7.9357);


	 neighbor -> 26
\draw[thick,dotted,gray] (9.37629,4.48826)--
(6.84629,7.36674);

\draw[thick,dotted,gray] (6.84629,7.36674)--
(3.45973,9.29528);


	 neighbor -> 0
\draw[ultra thick,dashed,red!50!yellow] (9.37629,4.48826)--
(8,5);

3 is expanded. 

	 neighbor -> 18
\draw[thick,dotted,gray] (9.78223,4.55585)--
(9.51248,3.48756);
	 neighbor -> 7
\draw[thick,dotted,gray] (9.78223,4.55585)--
(8.68801,3.30839);

	 neighbor -> 20
\draw[thick,dotted,gray] (9.78223,4.55585)--
(9.57914,1.79577);
	 neighbor -> 23
\draw[thick,dotted,gray] (9.78223,4.55585)--
(9.86223,7.9357);

	 neighbor -> 0
\draw[ultra thick,dashed,red!50!yellow] (9.78223,4.55585)--
(8,5);

18 is expanded. 
	 neighbor -> 7
\draw[thick,dotted,gray] (9.51248,3.48756)--
(8.68801,3.30839);


	 neighbor -> 20
\draw[thick,dotted,gray] (9.51248,3.48756)--
(9.57914,1.79577);
	 neighbor -> 0
\draw[ultra thick,dashed,red!50!yellow] (9.51248,3.48756)--
(8,5);

7 is expanded. 
	 neighbor -> 18
\draw[thick,dotted,gray] (8.68801,3.30839)--
(9.51248,3.48756);


	 neighbor -> 20
\draw[thick,dotted,gray] (8.68801,3.30839)--
(9.57914,1.79577);


	 neighbor -> 23
\draw[thick,dotted,gray] (8.68801,3.30839)--
(9.86223,7.9357);
	 neighbor -> 0
\draw[ultra thick,dashed,red!50!yellow] (8.68801,3.30839)--
(8,5);



29 is expanded. 

	 neighbor -> 22
\draw[ultra thick,dashed,red!50!yellow] (5.57414,8.68532)--
(2.8272,9.20994);
neighbor -> 12
\draw[ultra thick,dashed,red!50!yellow] (5.57414,8.68532)--
(2.54894,8.51295);
\draw[thick,green] (5.57414,8.68532)--
(2.54894,8.51295);
\draw[ thick,green] (2.62584,7.50763)--
(2.54894,8.51295);
\draw[ thick,green] (2.62584,7.50763)--
(2,5);
\draw[ultra thick,dashed,red!50!yellow] (2.62584,7.50763)--
(2.54894,8.51295);



	 neighbor -> 11
\draw[ultra thick,red!50!yellow] (5.57414,8.68532)--
(2.62584,7.50763);

\draw[ultra thick,magenta] (5.57414,8.68532)--
(2.62584,7.50763);
\draw[ultra thick,magenta] (2.62584,7.50763)--
(5.57414,8.68532);
\draw[ultra thick,magenta] (2.62584,7.50763)--
(1.53739,6.49119);
\draw[ultra thick,magenta] (2,5)--
(1.53739,6.49119);
\draw[ultra thick,magenta] (8,5)--
(6.72317,6.94032);
\draw[thick,green] (8,5)--
(6.72317,6.94032);
\draw[ultra thick,magenta] (6.72317,6.94032)--
(5.57414,8.68532);
\draw[thick,green] (6.72317,6.94032)--
(5.57414,8.68532);

\filldraw[black] (2.27339,3.18972)circle(2pt);
%\node[anchor=west] at(2.27339,3.18972){\scalebox{1}{$2$}}; 
\filldraw[black] (9.78223,4.55585)circle(2pt);
%\node[anchor=west] at(9.78223,4.55585){\scalebox{1}{$3$}}; 
\filldraw[black] (3.08013,2.63871)circle(2pt);
%\node[anchor=west] at(3.08013,2.63871){\scalebox{1}{$4$}}; 
\filldraw[black] (0.867434,4.19372)circle(2pt);
%\node[anchor=west] at(0.867434,4.19372){\scalebox{1}{$5$}}; 
\filldraw[black] (0.159104,5.27765)circle(2pt);
%\node[anchor=west] at(0.159104,5.27765){\scalebox{1}{$6$}}; 
\filldraw[black] (8.68801,3.30839)circle(2pt);
%\node[anchor=west] at(8.68801,3.30839){\scalebox{1}{$7$}}; 
\filldraw[black] (3.92942,6.7433)circle(2pt);
%\node[anchor=west] at(3.92942,6.7433){\scalebox{1}{$8$}}; 
\filldraw[black] (6.72317,6.94032)circle(2pt);
%\node[anchor=west] at(6.72317,6.94032){\scalebox{1}{$9$}}; 
\filldraw[black] (3.45973,9.29528)circle(2pt);
%\node[anchor=west] at(3.45973,9.29528){\scalebox{1}{$10$}}; 
\filldraw[black] (2.62584,7.50763)circle(2pt);
\node[anchor=west] at(2.62584,7.50763){\scalebox{1}{$11$}}; 
\filldraw[black] (2.54894,8.51295)circle(2pt);
%\node[anchor=west] at(2.54894,8.51295){\scalebox{1}{$12$}}; 
\filldraw[black] (1.74053,7.90764)circle(2pt);
%\node[anchor=west] at(1.74053,7.90764){\scalebox{1}{$13$}}; 
\filldraw[black] (9.37629,4.48826)circle(2pt);
%\node[anchor=west] at(9.37629,4.48826){\scalebox{1}{$14$}}; 
\filldraw[black] (3.8465,3.57475)circle(2pt);
%\node[anchor=west] at(3.8465,3.57475){\scalebox{1}{$15$}}; 
\filldraw[black] (1.93356,1.00474)circle(2pt);
%\node[anchor=west] at(1.93356,1.00474){\scalebox{1}{$16$}}; 
\filldraw[black] (4.82637,6.13703)circle(2pt);
%\node[anchor=west] at(4.82637,6.13703){\scalebox{1}{$17$}}; 
\filldraw[black] (9.51248,3.48756)circle(2pt);
%\node[anchor=west] at(9.51248,3.48756){\scalebox{1}{$18$}}; 
\filldraw[black] (2.76515,4.46506)circle(2pt);
\node[anchor=west] at(2.76515,4.46506){\scalebox{1}{$19$}}; 
\filldraw[black] (9.57914,1.79577)circle(2pt);
%\node[anchor=west] at(9.57914,1.79577){\scalebox{1}{$20$}}; 
\filldraw[black] (1.42716,0.835081)circle(2pt);
%\node[anchor=west] at(1.42716,0.835081){\scalebox{1}{$21$}}; 
\filldraw[black] (2.8272,9.20994)circle(2pt);
%\node[anchor=west] at(2.8272,9.20994){\scalebox{1}{$22$}}; 
\filldraw[black] (9.86223,7.9357)circle(2pt);
%\node[anchor=west] at(9.86223,7.9357){\scalebox{1}{$23$}}; 
\filldraw[black] (3.43305,3.00339)circle(2pt);
%\node[anchor=west] at(3.43305,3.00339){\scalebox{1}{$24$}}; 
\filldraw[black] (6.56972,2.59136)circle(2pt);
%\node[anchor=west] at(6.56972,2.59136){\scalebox{1}{$25$}}; 
\filldraw[black] (6.84629,7.36674)circle(2pt);
%\node[anchor=west] at(6.84629,7.36674){\scalebox{1}{$26$}}; 
\filldraw[black] (4.89423,9.53991)circle(2pt);
%\node[anchor=west] at(4.89423,9.53991){\scalebox{1}{$27$}}; 
\filldraw[black] (1.53739,6.49119)circle(2pt);
\node[anchor=west] at(1.53739,6.49119){\scalebox{1}{$28$}}; 
\filldraw[black] (5.57414,8.68532)circle(2pt);
%\node[anchor=west] at(5.57414,8.68532){\scalebox{1}{$29$}}; 
\filldraw[black] (1.43628,4.47904)circle(2pt);
\node[anchor=west] at(1.43628,4.47904){\scalebox{1}{$30$}}; 
\filldraw[black] (6.59233,6.6171)circle(2pt);
%\node[anchor=west] at(6.59233,6.6171){\scalebox{1}{$31$}}; 
   \filldraw[green] (2,5) circle(3pt);
\node[anchor=north] at(2,5) {\scalebox{0.9}{$(0.2,0.5)$}};
\node[anchor=north] at(8,5) {\scalebox{0.9}{$(0.8,0.5)$}};
\filldraw[red] (8,5) circle(3pt); 
\end{tikzpicture}   \label{fig:EIT*}
}
}
    \subfloat[Bidirectional Heuristic(BiIT*)]{
    \scalebox{0.38}{
\begin{tikzpicture}  
      %\filldraw[green!20] (1,2) -- (6,2) -- (6,0)--(3,0) --cycle; 
           %\filldraw[blue!20] (4,1) -- (6,1/3) -- (6,0)--(4,0) --cycle; 
     %\draw[step=1cm,gray,ultra thick](0,0) %grid(10,10);
     %\foreach \x in {0,...,10}
       %\draw (\x cm,1pt) -- (\x cm,-1pt) node[anchor=north] {$\x$};
       %\foreach \y in {1,...,10}
        %\draw (1pt,\y cm) -- (-1pt,\y cm) node[anchor=east] {$\y$};
%\filldraw[color=red!60, fill=red!5, very ultra thick](5,5) circle (2.5);
\draw[ultra thick] (0,0) -- (10,0) node[anchor=north west]{};
\draw[ultra thick] (0,0) -- (0,10) node[anchor=south east]{};
\draw[ultra thick] (0,10) -- (10,10) node[anchor=south east]{};
\draw[ultra thick] (10,0) -- (10,10) node[anchor=south east]{};
\filldraw[gray, ultra thick](4,0) rectangle (6,5.8);
\filldraw[gray, ultra thick](4,6.2) rectangle (6,8);
\filldraw[gray, ultra thick](4,0) rectangle (6,5.8);


0 is expanded. 
	 neighbor -> 14
\draw[thick,dotted,gray] (8,5)--
(9.37629,4.48826);
	 neighbor -> 7
\draw[thick,dotted,gray] (8,5)--
(8.68801,3.30839);
	 neighbor -> 3
\draw[thick,dotted,gray] (8,5)--
(9.78223,4.55585);
	 neighbor -> 18
\draw[thick,dotted,gray] (8,5)--
(9.51248,3.48756);
	 neighbor -> 31
\draw[thick,dotted,gray] (8,5)--
(6.59233,6.6171);
	 neighbor -> 9
\draw[thick,dotted,gray] (8,5)--
(6.72317,6.94032);
	 neighbor -> 26
\draw[thick,dotted,gray] (8,5)--
(6.84629,7.36674);
	 neighbor -> 25
\draw[thick,dotted,gray] (8,5)--
(6.56972,2.59136);
	 neighbor -> 17
\draw[thick,dotted,gray] (8,5)--
(4.82637,6.13703);
	 neighbor -> 23
%\draw[ultra thick,dashed,red!50!yellow] (8,5)--(9.86223,7.9357);

1 is expanded. 
	 neighbor -> 30
\draw[thick,dotted,gray] (2,5)--
(1.43628,4.47904);
	 neighbor -> 19
\draw[thick,dotted,gray] (2,5)--
(2.76515,4.46506);
	 neighbor -> 5
\draw[thick,dotted,gray] (2,5)--
(0.867434,4.19372);
	 neighbor -> 28
\draw[thick,dotted,gray] (2,5)--
(1.53739,6.49119);
	 neighbor -> 2
\draw[thick,dotted,gray] (2,5)--
(2.27339,3.18972);
	 neighbor -> 6
\draw[thick,dotted,gray] (2,5)--
(0.159104,5.27765);
	 neighbor -> 15
\draw[thick,dotted,gray] (2,5)--
(3.8465,3.57475);
	 neighbor -> 24
\draw[thick,dotted,gray] (2,5)--
(3.43305,3.00339);
	 neighbor -> 11
\draw[thick,dotted,gray] (2,5)--
(2.62584,7.50763);
	 neighbor -> 4
\draw[thick,dotted,gray] (2,5)--
(3.08013,2.63871);
	 neighbor -> 8
\draw[thick,dotted,gray] (2,5)--
(3.92942,6.7433);
	 neighbor -> 13
\draw[thick,dotted,gray] (2,5)--
(1.74053,7.90764);
	 neighbor -> 17
\draw[thick,dotted,gray] (8,5)--
(9.86223,7.9357);
%\draw[ultra thick,dashed,red!50!yellow] (8,5)--(4.82637,6.13703);


1  19
19 is expanded. 

	 neighbor -> 30
%\draw[ultra thick,dashed,red!50!yellow] (2.76515,4.46506)--(1.43628,4.47904);
	 neighbor -> 2
%\draw[ultra thick,dashed,red!50!yellow] (2.76515,4.46506)--(2.27339,3.18972);
	 neighbor -> 15
\draw[thick,dotted,gray] (2.76515,4.46506)--
(3.8465,3.57475);
	 neighbor -> 24
\draw[thick,dotted,gray] (2.76515,4.46506)--
(3.43305,3.00339);
	 neighbor -> 4
\draw[thick,dotted,gray] (2.76515,4.46506)--
(3.08013,2.63871);
	 neighbor -> 5
%\draw[ultra thick,,dashed,red!50!yellow] (2.76515,4.46506)--(0.867434,4.19372);
	 neighbor -> 28
\draw[ultra thick,dashed,red!40!blue] (3.92942,6.7433)--
(1.53739,6.49119);
	 neighbor -> 8
\draw[thick,dotted,gray] (2.76515,4.46506)--
(3.92942,6.7433);
	 neighbor -> 17
\draw[thick,dotted,gray] (2.76515,4.46506)--
(4.82637,6.13703);

	 neighbor -> 17
\draw[ultra thick,dashed,red!40!blue] (2.76515,4.46506)--
(4.82637,6.13703);
	 neighbor -> 17
\draw[ultra thick,dashed,red!40!blue] (3.92942,6.7433)--
(4.82637,6.13703);
	 neighbor -> 15
\draw[ultra thick,dashed,red!40!blue] (4.82637,6.13703)--
(3.8465,3.57475);


17 is expanded. 
	 neighbor -> 31
\draw[ultra thick,dashed,red!50!yellow] (4.82637,6.13703)--
(6.59233,6.6171);
	 neighbor -> 9
\draw[ultra thick,dashed,red!50!yellow] (4.82637,6.13703)--
(6.72317,6.94032);
	 neighbor -> 26
\draw[ultra thick,dashed,red!50!yellow] (4.82637,6.13703)--
(6.84629,7.36674);
	 neighbor -> 11
\draw[ultra thick,dashed,red!40!blue] (4.82637,6.13703)--
(2.62584,7.50763);
	 neighbor -> 29
\draw[ultra thick,dashed,red!50!yellow] (4.82637,6.13703)--(5.57414,8.68532);
	 neighbor -> 15
\draw[thick,dashed,gray] (4.82637,6.13703)--
(3.8465,3.57475);
	 neighbor -> 1
\draw[ultra thick,dashed,red!50!yellow] (4.82637,6.13703)--
(2,5);
	 neighbor -> 12
\draw[ultra thick,dashed,red!40!blue] (4.82637,6.13703)--(2.54894,8.51295);
	 neighbor -> 0
\draw[ultra thick,dashed,red!40!blue] (4.82637,6.13703)--
(8,5);

	 neighbor -> 9
\draw[thick,dotted,gray] (6.59233,6.6171)--
(6.72317,6.94032);
	 neighbor -> 26
\draw[thick,dotted,gray] (6.59233,6.6171)--
(6.84629,7.36674);
	 neighbor -> 17
\draw[thick,dotted,gray] (6.59233,6.6171)--
(4.82637,6.13703);
	 neighbor -> 0
\draw[thick,dotted,gray] (6.59233,6.6171)--
(8,5);
	 neighbor -> 29
\draw[thick,dotted,gray] (6.59233,6.6171)--
(5.57414,8.68532);
	 neighbor -> 8
\draw[thick,dotted,gray] (6.59233,6.6171)--
(3.92942,6.7433);

	 neighbor -> 14
\draw[thick,dotted,gray] (6.59233,6.6171)--
(9.37629,4.48826);
	 neighbor -> 23
\draw[thick,dotted,gray] (6.59233,6.6171)--
(9.86223,7.9357);
	 neighbor -> 3
\draw[thick,dotted,gray] (6.59233,6.6171)--
(9.78223,4.55585);
	 neighbor -> 7
\draw[thick,dotted,gray] (6.59233,6.6171)--
(8.68801,3.30839);
	 neighbor -> 25
\draw[thick,dotted,gray] (6.59233,6.6171)--
(6.56972,2.59136);

	 neighbor -> 0
\draw[thick,dotted,gray] (6.59233,6.6171)--
(8,5);

%\draw[ultra thick,dashed,red!50!yellow] (8,5)--(6.59233,6.6171);

9 is expanded. 


	 neighbor -> 23
\draw[thick,dotted,gray] (6.72317,6.94032)--
(9.86223,7.9357);
	 neighbor -> 14
\draw[thick,dotted,gray] (6.72317,6.94032)--
(9.37629,4.48826);
	 neighbor -> 3
\draw[thick,dotted,gray] (6.72317,6.94032)--
(9.78223,4.55585);


%\draw[ultra thick,dashed,red!50!yellow] (6.72317,6.94032)--(8,5);

25 is expanded. 
	 neighbor -> 7
\draw[thick,dotted,gray] (6.56972,2.59136)--
(8.68801,3.30839);

	 neighbor -> 18
\draw[thick,dotted,gray] (6.56972,2.59136)--
(9.51248,3.48756);
	 neighbor -> 20
\draw[thick,dotted,gray] (6.56972,2.59136)--
(9.57914,1.79577);

	 neighbor -> 14
\draw[thick,dotted,gray] (6.56972,2.59136)--
(9.37629,4.48826);

	 neighbor -> 3
\draw[thick,dotted,gray] (6.56972,2.59136)--
(9.78223,4.55585);

	 neighbor -> 31
\draw[thick,dotted,gray] (6.56972,2.59136)--
(6.59233,6.6171);

	 neighbor -> 0
%\draw[ultra thick,dashed,red!50!yellow] (6.56972,2.59136)--(8,5);

26 is expanded. 

	 neighbor -> 29
\draw[thick,dotted,gray] (6.84629,7.36674)--
(5.57414,8.68532);


	 neighbor -> 27
\draw[thick,dotted,gray] (6.84629,7.36674)--
(4.89423,9.53991);

	 neighbor -> 23
\draw[thick,dotted,gray] (6.84629,7.36674)--
(9.86223,7.9357);


	 neighbor -> 0
%\draw[ultra thick,,dashed,red!50!yellow] (6.84629,7.36674)--(8,5);

14 is expanded. 

	 neighbor -> 18
\draw[thick,dotted,gray] (9.37629,4.48826)--
(9.51248,3.48756);
	 neighbor -> 7
\draw[thick,dotted,gray] (9.37629,4.48826)--
(8.68801,3.30839);

	 neighbor -> 20
\draw[thick,dotted,gray] (9.37629,4.48826)--
(9.57914,1.79577);

	 neighbor -> 23
\draw[thick,dotted,gray] (9.37629,4.48826)--
(9.86223,7.9357);


	 neighbor -> 26
\draw[thick,dotted,gray] (9.37629,4.48826)--
(6.84629,7.36674);

\draw[thick,dotted,gray] (6.84629,7.36674)--
(3.45973,9.29528);


	 neighbor -> 0
%\draw[ultra thick,dashed,red!50!yellow] (9.37629,4.48826)--(8,5);

3 is expanded. 

	 neighbor -> 18
\draw[thick,dotted,gray] (9.78223,4.55585)--
(9.51248,3.48756);
	 neighbor -> 7
\draw[thick,dotted,gray] (9.78223,4.55585)--
(8.68801,3.30839);

	 neighbor -> 20
\draw[thick,dotted,gray] (9.78223,4.55585)--
(9.57914,1.79577);
	 neighbor -> 23
\draw[thick,dotted,gray] (9.78223,4.55585)--
(9.86223,7.9357);

	 neighbor -> 0
%\draw[ultra thick,dashed,red!50!yellow] (9.78223,4.55585)--
(8,5);

18 is expanded. 
	 neighbor -> 7
\draw[thick,dotted,gray] (9.51248,3.48756)--
(8.68801,3.30839);


	 neighbor -> 20
\draw[thick,dotted,gray] (9.51248,3.48756)--
(9.57914,1.79577);
	 neighbor -> 0
%\draw[ultra thick,dashed,red!50!yellow] (9.51248,3.48756)--
(8,5);

7 is expanded. 
	 neighbor -> 18
\draw[thick,dotted,gray] (8.68801,3.30839)--
(9.51248,3.48756);


	 neighbor -> 20
\draw[thick,dotted,gray] (8.68801,3.30839)--
(9.57914,1.79577);


	 neighbor -> 23
\draw[thick,dotted,gray] (8.68801,3.30839)--
(9.86223,7.9357);
	 neighbor -> 0
%\draw[ultra thick,dashed,red!50!yellow] (8.68801,3.30839)--
(8,5);



29 is expanded. 

	 neighbor -> 22
%\draw[ultra thick,dashed,red!50!yellow] (5.57414,8.68532)--(2.8272,9.20994);
	 neighbor -> 12
%\draw[ultra thick,dashed,red!50!yellow] (5.57414,8.68532)--
%(2.54894,8.51295);
	 neighbor -> 11
%\draw[ultra thick,red!50!yellow] (5.57414,8.68532)--(2.62584,7.50763);

\draw[ultra thick,blue] (5.57414,8.68532)--
(2.62584,7.50763);
\draw[ultra thick,blue] (2.62584,7.50763)--
(5.57414,8.68532);
\draw[ultra thick,blue] (2.62584,7.50763)--
(2,5);

\draw[ultra thick,blue] (8,5)--
(6.72317,6.94032);
\draw[ultra thick,blue] (6.72317,6.94032)--
(5.57414,8.68532);

\filldraw[black] (2.27339,3.18972)circle(2pt);
%\node[anchor=west] at(2.27339,3.18972){\scalebox{1}{$2$}}; 
\filldraw[black] (9.78223,4.55585)circle(2pt);
%\node[anchor=west] at(9.78223,4.55585){\scalebox{1}{$3$}}; 
\filldraw[black] (3.08013,2.63871)circle(2pt);
%\node[anchor=west] at(3.08013,2.63871){\scalebox{1}{$4$}}; 
\filldraw[black] (0.867434,4.19372)circle(2pt);
%\node[anchor=west] at(0.867434,4.19372){\scalebox{1}{$5$}}; 
\filldraw[black] (0.159104,5.27765)circle(2pt);
%\node[anchor=west] at(0.159104,5.27765){\scalebox{1}{$6$}}; 
\filldraw[black] (8.68801,3.30839)circle(2pt);
%\node[anchor=west] at(8.68801,3.30839){\scalebox{1}{$7$}}; 
\filldraw[black] (3.92942,6.7433)circle(2pt);
%\node[anchor=west] at(3.92942,6.7433){\scalebox{1}{$8$}}; 
\filldraw[black] (6.72317,6.94032)circle(2pt);
%\node[anchor=west] at(6.72317,6.94032){\scalebox{1}{$9$}}; 
\filldraw[black] (3.45973,9.29528)circle(2pt);
%\node[anchor=west] at(3.45973,9.29528){\scalebox{1}{$10$}}; 
\filldraw[black] (2.62584,7.50763)circle(2pt);
%\node[anchor=west] at(2.62584,7.50763){\scalebox{1}{$11$}}; 
\filldraw[black] (2.54894,8.51295)circle(2pt);
%\node[anchor=west] at(2.54894,8.51295){\scalebox{1}{$12$}}; 
\filldraw[black] (1.74053,7.90764)circle(2pt);
%\node[anchor=west] at(1.74053,7.90764){\scalebox{1}{$13$}}; 
\filldraw[black] (9.37629,4.48826)circle(2pt);
%\node[anchor=west] at(9.37629,4.48826){\scalebox{1}{$14$}}; 
\filldraw[black] (3.8465,3.57475)circle(2pt);
%\node[anchor=west] at(3.8465,3.57475){\scalebox{1}{$15$}}; 
\filldraw[black] (1.93356,1.00474)circle(2pt);
%\node[anchor=west] at(1.93356,1.00474){\scalebox{1}{$16$}}; 
\filldraw[red!50!green] (4.82637,6.13703)circle(2pt);
%\node[anchor=west] at(4.82637,6.13703){\scalebox{1}{$17$}}; 
\filldraw[black] (9.51248,3.48756)circle(2pt);
%\node[anchor=west] at(9.51248,3.48756){\scalebox{1}{$18$}}; 
\filldraw[black] (2.76515,4.46506)circle(2pt);
%\node[anchor=west] at(2.76515,4.46506){\scalebox{1}{$19$}}; 
\filldraw[black] (9.57914,1.79577)circle(2pt);
%\node[anchor=west] at(9.57914,1.79577){\scalebox{1}{$20$}}; 
\filldraw[black] (1.42716,0.835081)circle(2pt);
%\node[anchor=west] at(1.42716,0.835081){\scalebox{1}{$21$}}; 
\filldraw[black] (2.8272,9.20994)circle(2pt);
%\node[anchor=west] at(2.8272,9.20994){\scalebox{1}{$22$}}; 
\filldraw[black] (9.86223,7.9357)circle(2pt);
%\node[anchor=west] at(9.86223,7.9357){\scalebox{1}{$23$}}; 
\filldraw[black] (3.43305,3.00339)circle(2pt);
%\node[anchor=west] at(3.43305,3.00339){\scalebox{1}{$24$}}; 
\filldraw[black] (6.56972,2.59136)circle(2pt);
%\node[anchor=west] at(6.56972,2.59136){\scalebox{1}{$25$}}; 
\filldraw[black] (6.84629,7.36674)circle(2pt);
%\node[anchor=west] at(6.84629,7.36674){\scalebox{1}{$26$}}; 
\filldraw[black] (4.89423,9.53991)circle(2pt);
%\node[anchor=west] at(4.89423,9.53991){\scalebox{1}{$27$}}; 
\filldraw[black] (1.53739,6.49119)circle(2pt);
%\node[anchor=west] at(1.53739,6.49119){\scalebox{1}{$28$}}; 
\filldraw[black] (5.57414,8.68532)circle(2pt);
%\node[anchor=west] at(5.57414,8.68532){\scalebox{1}{$29$}}; 
\filldraw[black] (1.43628,4.47904)circle(2pt);
%\node[anchor=west] at(1.43628,4.47904){\scalebox{1}{$30$}}; 
\filldraw[black] (6.59233,6.6171)circle(2pt);
%\node[anchor=west] at(6.59233,6.6171){\scalebox{1}{$31$}}; 
   \filldraw[green] (2,5) circle(3pt);
%\node[anchor=west] at(2,5) {$S$};
%\node[anchor=west] at(8,5) {$G$};
\node[anchor=north] at(8,5){\scalebox{0.9}{$(0.8,0.5)$}}; 
\node[anchor=north] at(2,5){\scalebox{0.9}{$(0.2,0.5)$}}; 
\filldraw[red] (8,5) circle(3pt); 
\end{tikzpicture} \label{fig:biit}
}
} 

\caption{\textbf{Admissibility of} the reverse search of EIT* and AIT* (\ref{fig:EIT*}) and the bidirectional search of BiIT* (\ref{fig:biit}). The green (\textcolor{green}{$\bullet$}) and the red  (\textcolor{red}{${\bullet}$}) denotes the start and goal states, respectively. A random geometric graph is built by implicit edges connected via gray (\textcolor{gray}{${\dots}$}) between any two informed states (\textcolor{black}{${\bullet}$}). The initial solution found by BIT* using Euclidean norm as its heuristic is shown in green ($\textcolor{green}{-}$) in (\ref{fig:EIT*}). The initial solutions found by AIT* and EIT* via adaptive heuristic are shown in green ($\textcolor{green}{-}$) and magenta ($\textcolor{magenta}{-}$) in (\ref{fig:EIT*}), respectively.  The initial solution found by BiIT* is shown in blue ($\textcolor{blue}{-}$) in (\ref{fig:biit}). In (\ref{fig:EIT*}), the heuristic provided from reverse tree of AIT* and EIT* is show in dashed orange($\textcolor{orange}{--}$). In (\ref{fig:biit}), the heuristic provided by lazy reverse search of BiIT* is shown in purple($\textcolor{purple}{--}$) while orange($\textcolor{orange}{--}$) presents the heuristic provided by the lazy forward search of BiIT*. (\ref{fig:EIT*}) and (\ref{fig:biit}) are obstained by running BIT*, EIT*, AIT*, and BiIT* on OMPL, where the seed ID: 7 and 30 samples per batch.}   
    \label{fig:EITandBiIT}
\end{figure} 


RRT-connect~\cite{rrtconect}, a bidirectional sampling-based planner, offers fast planning performance and works well in a high dimensional continuous state space. 

 We sketch the reasons as follows: 
 
 \textbf{Mutuality of k-nearest neighbors:} Arguably, it can barely guarantee the mutuality of k-nearest neighbors when building RGGs on-the-fly with uniform sampling. Suppose the edges are connected by $k$-$\mathit{nearest}$ neighbors. For a connected edge $(\mathbf{s,v})$ when searching forward, it cannot ensure $\mathbf{s}$ is one of the $k$-nearest neighbor of $\mathbf{v}$ when searching reverse due to uniform sampling. Thus, $\mathbf{s}$ cannot guarantee to get the admissible $cost$-$to$-$go$ if $\widehat{h}(\mathbf{v})$ is admissible on the reverse search of AIT* or EIT*. 
 
 \textbf{R-disc connection or mutual k-nearest neighbors:} Suppose the edges are connected either by a $\mathit{radius}$ or a mutual $k$-$\mathit{nearest}$ neighbors. The lazy reverse search of AIT* and EIT* is a version of A* to update heuristic from the goal state to all generated states, where the reverse tree of EIT* is an edge-queue version of A* with adaptive sparse collision detection~\cite{EIT}. However, A* can only guarantee the optimal $cost$-$to$-$come$ for each expanded vertex but not for those vertices that had been generated but had yet to be expanded~\cite{A*}~\cite{Pearl}. Accordingly, AIT* and EIT* cannot guarantee the admissibility by their reverse searching because the reverse search does not actually check collision between those implicit edges. For example, $\widehat{h}[11]=\infty$ when EIT* generates 11, where $\widehat{h}[\cdot]$ denotes the calculated admisible cost heuristic in~\cite{EIT} .
 
 %For example, In Figure~\ref{fig:EIT*}, heuristic value of the state 11 is updated by the reverse tree,  $\widehat{h}(11) =\infty$, that represents inadmissible, when EIT* selected 28 for expansion. 


  $E_\mathcal{F} = \{(\mathbf{u}_{\mathcal{F}},\mathbf{v}_{\mathcal{F}} ) | \{\mathbf{u}_{\mathcal{F}},\mathbf{v}_{\mathcal{F}}\} \in V_{\mathcal{F}} \}$





  
  
 
 Unlike AIT* that providing a more accurate heuristic via reverse search, EIT* supplies an admissible heuristic, an inadmissible heuristic, and an inadmissible effort heuristic, where the reverse search of EIT* is with adaptive sparse collision checking. However, the reverse search cannot ensure providing an admissible heuristic. An inadmissible heuristic could result the search in getting trapped in the reverse search, which leads to more edges for collision checks.

 AIT* and EIT*~\cite{EIT}, asymmetric bidirectional optimal sampling-based motion planners, provide an accurate heuristic by using an inexpensive reverse search for their forward search. Unlike AIT* that providing a more accurate heuristic via reverse search, EIT* supplies an admissible heuristic, an inadmissible heuristic, and an inadmissible effort heuristic, where the reverse search of EIT* is with adaptive sparse collision checking. However, the reverse search cannot ensure providing an admissible heuristic. An inadmissible heuristic could result the search in getting trapped in the reverse search, which leads to more edges for collision checks.

 , an asymmetric bidirectional sampling-based motion planner,

 It firstly employs a bidirectional heuristic search (without collision checks) and uniform-cost search (), such as MM~\cite{mm} and Dijkstra's algorithm~\cite{dijstra}, to provide a precise and an admissible heuristic for an given RGG. Then it runs a bidirectional heuristic search in both direction with the provided admissible heuristic.  BiIT* maintains the anytime fashion on each batch, which similarly runs BIT* in both direction with the provided heuristic.    

  Whenever a state $\mathbf{s}$ actives the stopping condition for the lazy bidirectional search (Algorithm1: Line13), BiIT* starts to update heuristic values for the states on either lazy forward search tree or reverse search tree separately by a lazy Dijkstra's algorithm with bounded estimated solutions (Algorithm~\ref{alg1}:Line15-16).

  updates the heuristic values for the generated states on the lazy forward search tree by using lazy Dijkstra's algorithm with the bounded estimated solution, the generated states on the lazy reverse search tree are processing analogously.

  An anytime sampling-based motion planning algorithm with an admissible heuristic is asymptotically optimal, as the total number of samples goes to infinity~\cite{AWA}~\cite{bit}. 


  With adaptive sparse collision checks, both admissible and inadmissible heuristics are obtained from the reverse search of EIT*. However, the inadmissible heuristic might be used by EIT* in the next-step forward search to find a solution. This can result in longer reverse search time, and further brings more collision checks for the edges.

 \begin{figure*}
  \vspace{-10mm}
    \centering 
    %\subfloat[]{
    %\scalebox{0.8}{
    %\includegraphics[width=55mm,scale=0.8]{BiIT.pdf}}}
       \subfloat[\scalebox{0.75}{Initial Solution Time ($\mathbb{R}^8$)}]{
    \scalebox{0.5}{
    \includegraphics[width=90mm,scale=0.7]{R8EnTIMEI.pdf}}}
    \subfloat[Initial Path Cost ($\mathbb{R}^8$)]{
    \scalebox{0.5}{
    \includegraphics[width=90mm,scale=0.7]{R8EnCostI.pdf}}
    }
    \subfloat[Final Path Cost ($\mathbb{R}^8$)]{
    \scalebox{0.5}{
    \includegraphics[width=90mm,scale=0.7]{R8EnCostF.pdf}}
    }
  %\vspace{-4mm}
       \subfloat[Initial Solution Time ($\mathbb{R}^{16}$)]{
    \scalebox{0.5}{
    \includegraphics[width=90mm,scale=0.7]{R16EnTime.pdf}}}
    \subfloat[Initial Path Cost ($\mathbb{R}^{16}$)]{
    \scalebox{0.5}{
    \includegraphics[width=90mm,scale=0.7]{R16EnCostI.pdf}}
    }
    \subfloat[Final Path Cost ($\mathbb{R}^{16}$)]{
    \scalebox{0.5}{
    \includegraphics[width=90mm,scale=0.7]{R16EnCostF.pdf}}
    }
    
    \caption{Compansions of initial and final search performance on Goal Enclosure with Wall Gap Map in $\mathbb{R}^8$ and $\mathbb{R}^{16}$ of BIT*, EIT* and BiIT*. We set cut =0 to restrict the violin range within the range of our testing data. The violin plots display the 95$\%$ confidence interval (lines that extend from the center). The violin plots show BiIT* outperforms BIT* and EIT* in faster finding an initial solution and improving the convergence. Note that the plot does not show BIT*'s performance because the successful runs are less than 50 trails in $\mathbb{R}^{16}$.}
    \label{fig:VPE}  
\end{figure*}



Anytime incremental graph-search algorithms combing the properties of anytime and incremental search, such as Anytime D* (AD*)~\cite{AD*} and Anytime Truncated D* (ATD*)~\cite{TA*}, can promptly return a first solution by a weighted heuristic, and then continually decrease the path cost with iteratively reducing the weighted factor. Meanwhile, the planners repair the incumbent solution once the searching graph is changed. 

  BiIT*, a new asymptotically optimal sampling-based motion planner, uses the strengths of bidirectional heuristic search, such as MM~\cite{mm}, and anytime informed sampling-based planners, such as BIT*~\cite{bit}, to find solutions on a given RGG until an optimal solution is found or time is not allowed any more. 

   EIT* and BiIT* are run drone for planning a path on UNH Campus Map. EIT* and BiIT* sample 6000 states per batch in this 2D terrain. We set $\eta = 1.001$, and 200 line-segments for collision checks between any two states for the tested planners. EIT* and BiIT* are run 100 trails and given 2 seconds for each trail. Fig.~\ref{unhanytime}  and Fig.~\ref{fig:VPUNH} show the comparison results between the two algorithms. The quadrotor is considered as a point robot in the mission, and it follows the planned waypoints consecutively. 
 
 
 The drone is with the  autopilot system (controller) and is used for a path planning mission. The drone has compact dimensions of $44\times84\times12$ mm, and the GPS input port of this drone for navigation is with the accuracy of approximately $\pm$2.5 m.

 As demonstrated on both simulated and real-world experiments, BIT* outperforms existing sampling-based optimal
planners and RRT, especially in high dimensions. For a
given computational time, BIT* has a higher likelihood of
finding a solution and generally finds solutions of equivalent
quality sooner. It also converges towards the optimum faster
than other asymptotic optimal planners, and has recently
been shown to perfo
 
 Accurate and admissible heuristics were guaranteed by using our method, and 

 An accurate and admissible heuristic is beneficial to improve the searching performance for an anytime sampling-based motion planner. In this paper, we present BiIT*, an asymptotically optimal sampling-based planner conducts by an precise and admissible heuristic to a problem instance. BiIT* applies an accurate and admissible heuristic provided by a bidirectional heuristic search (without collision checks) and Dijkstra's algorithm to guide a bidirectional search. BiIT* outperforms EIT*, the state-of-art sampling-based motion planner, on the measured abstract problems and UNH Campus Map in finding a first solution and convergence of the optima. 

 %BiIT* and EIT* have no advantages on maps that lack large local minima: \url{https://movingai.com/benchmarks/dao/orz100d.svg} but BIT* works well. One of the future work is to improve BiIT* to solve this problem.  

In the real world, an environment is usually unpredictable, involving in moving obstacles and unknown scenes, a rapid replanning method is needed to find a safe path. 





The recent  advances in incremental motion planners, such as 
ATD*~\cite{TA*}, RRT$^X$~\cite{rrtx}, and Lifelong-GLS\cite{lim2022lazy} have significantly prompt the searching efficiency in a dynamic environment, yet these planners either require an offline computation of a lattice graph or pre-built a topology graph, or needs expensive edge computations for each potentially valid edge. Therefore, there still needs an anytime online sampling-based replanner that can reduce large amount of collision checks by an accurate and admissible heuristic without offline computations in an uncertain environment. We will direct future work toward delivering an anytime single-query sampling-based kinodynamic motion planning algorithm with fast replanning.  

%The planners also pre-define a weight.
RRT$^X$~\cite{rrtx}, the first real-time sampling-based replanning algorithm, can efficiently replan in a dynamic environment without any precomputing processing. But it still . 

Once the above mentioned stop condition is satisfied, BiIT* begins to update the heuristic in both search trees by a uniform-cost search, such as Dijkstra's algorithm, from the $meeting~state$ $\mathbf{s}$ towards $X_{start}$ and $X_{goal}$, respectively (Alg.~\ref{alg1}, line 15-16, and Alg.~\ref{alg2}). In this process, we provide a bound 
